Deep joint source-channel coding for wireless point cloud transmission

The growing demand for high-quality point cloud transmission over wireless networks presents significant challenges, primarily due to the large data sizes and the need for efficient encoding techniques. In response to these challenges, we introduce a novel system named Deep Point Cloud Semantic Transmission (PCST), designed for end-to-end wireless point cloud transmission. Our approach employs a progressive resampling framework using sparse convolution to project point cloud data into a semantic latent space. These semantic features are subsequently encoded through a deep joint source-channel (JSCC) encoder, generating the channel-input sequence. To enhance transmission efficiency, we use an adaptive entropy-based approach to assess the importance of each semantic feature, allowing transmission lengths to vary according to their predicted entropy. PCST is robust across diverse Signal-to-Noise Ratio (SNR) levels and supports an adjustable rate-distortion (RD) trade-off, ensuring flexible and efficient transmission. Experimental results indicate that PCST significantly outperforms traditional separate source-channel coding (SSCC) schemes, delivering superior reconstruction quality while achieving over a 50% reduction in bandwidth usage.

==> copy/method_copy.tex <==
The sixth generation (6G) mobile network is expected to deliver  high-speed and high-efficiency transmission for different applications. Point cloud enabled virtual reality/augmented reality (VR/AR) is regarded as one of the most important high-throughput application-level requirements for 6G. Unlike image and video, point clouds demand substantial bandwidth for reliable transmission. To address this challenge, current methods typically involves two key steps: source coding and channel coding. Source coding methods aim to compress the source into smaller bit sizes. Notably, current representative standard methods are Geometry-based Point Cloud Compression (GPCC) and Video-based Point Cloud Compression (VPCC). In contrast, channel coding methods, such as such as Low-Density Parity-Check (LDPC) and Polar coding, add redundant bits to facilitate error correction and protect the transmission quality. However, one significant issue arises from the variable nature of wireless channel, leading to the cliff effect in separation-based schemes, where the performance breaks down when the capacity falls below the current communication rate. 

Semantic transmission with joint source and channel coding (JSCC) schemes has proven effective in mitigating the cliff effect, as the end-to-end structure can be trained under channel noise. This method has been extensively studied in the context of image, speech, and video transmission. However, research on point cloud transmission remains sparse due to the large size and complexity of point cloud data.

In this paper, we propose point cloud semantic transmission (PCST) model, which is trained to adapt to both additive white Gaussian noise (AWGN) and Rayleigh channels. Our contributions are three-fold:


1. To the best of our knowledge, this is the first paper to investigate semantic point cloud transmission. We propose the PCST model to efficiently compress geometry-based point cloud information.

2. To adapt to different available bandwidth, we propose a Deep JSCC module with switchable FC layers. This module translates symbols to different sizes, ensuring efficient use of the available bandwidth.

3. Numerical results verify the performance of PCST across both AWGN and Rayleigh channels. Compared with classical separate schemes \textit{GPCC + LDPC} and \textit{VPCC + LDPC}. Great performance can obtained across D1 PSNR. With a similar objective score, our model can save up to xxx\% of the bandwidth cost.

Through these contributions, our proposed PCST model aims to enhance the efficiency and reliability of point cloud transmission in future networks.







\subsection{Architecture}
The proposed PCST model comprises a semantic feature network, a Deep Joint Source-Channel Coding (Deep JSCC) codec, and an entropy model. The point cloud information $X$ is represented as a sparse tensor ${C_X, F_X}$, where $C_X$ denotes the coordinates of the point cloud and $F_X$ is an all-ones vector. Initially, the point cloud information $X$ is processed through the encoder $c_e$ with multiple down-sampling operations to obtain the latent feature $Y$. $Y$ is then quantized into $\Tilde{Y}$ and fed into both entropy model and Deep JSCC encoder. The entropy model first calculate feature entropy to determine the semantic importance of $Y$; Based on this importance, $Y$ is processed through corresponding Deep JSCC encoders and be transformed into a symbol sequence $\mathbf{S}$. $\mathbf{S}$ is then transmitted through a wireless channel, donated as $W(S|h)$, where $h$ represents the channel state information (CSI). In this paper, we consider both Additive White Gaussian Noise (AWGN) and Rayleigh channels. If a Rayleigh channel is chosen, the symbols will pass through a channel equalizer before decoding. The received symbols are donated as $\hat{\mathbf{S}}$. The decoding networks utilize a mirror architecture of the encoding networks. The decoding process begins with $f_d$ to retrieve the latent feature $\hat{Y}$, followed by $c_d$ with transposed convolution and binary classification to restore $\hat{X}$. Throughout the transmission process, the side information includes the number of points in each round of down-sampling during fearure extraction and the coordinates of $Y$. This side information should be transmitted via reliable digital transmission and is relatively small compared to $S$.


\begin{equation}
X \xrightarrow{c_e(\cdot)} Y \xrightarrow{Q(\cdot)} \Tilde{Y}\xrightarrow{f_e(\cdot)} S \xrightarrow{W(\cdot|h)} \hat{S} \xrightarrow{f_d(\cdot)} \hat{Y} \xrightarrow{c_d(\cdot)} \hat{X}
\end{equation}

\begin{equation}
\quad Y \xrightarrow{e(\cdot)} \{\mu, \sigma\} \xrightarrow{g(\cdot)} k.
\end{equation}

\subsection{Rate distortion}

In this paper, we address the allocation of latent features with varying bandwidths according to their respective importance. We propose an entropy model to estimate the distribution of $Y$, adaptively adjust the symbol sizes to meet the available bandwidth.

We assume the latent feature $Y$ follows a Gaussian Mixture Model (GMM) distribution $\mathcal{N}(\mu_i, \sigma_i^2)$. The parameters of the distribution can be estimated by a fully factorized model. The training process can be formulated as:
\begin{equation}
    p_{y|\psi}(y|\psi) = \prod_{i} \left( p_{y_i|\psi_{(i)}}(\psi^{(i)}) * \mathcal{U}\left(-\frac{1}{2}, \frac{1}{2}\right) \right)(y_i),
\end{equation}

where $*$ is the convolution operation, $p_{y|\psi}(y|\psi)$ represents the conditional probability of $Y$ given $\phi$, and $\mathcal{U}\left(-\frac{1}{2}, \frac{1}{2}\right) $ denotes the uniform distribution. 

The channel bandwidth cost $K$ can be derived from this probability, as follows: 
\begin{equation}
    K=\sum_i k_i=\sum_i-\eta_i\log_2 P(F_{Y}),
\end{equation}
where $\eta_i$ represents the proportion from latent feature $y_i$ to the number of symbols.
\subsection{Optimization goal} 
The overall loss function is defined as:
\begin{equation}
    J_{loss}=R+\lambda D=\sum_{i=1}^{N} k_i + \lambda D,
\end{equation}
where $R$ represents the bandwidth cost and D denotes the distortion.The distortion $D$ is calculated using the Binary Cross-Entropy (BCE) loss:
\begin{equation}
    D=\frac{1}{N}\sum_i -(x_i \log (p_i)+(1-x_i)\log(1-p_i)),
\end{equation}
where $x_i$ is the true value, $p_i$ is the predicted probability,
R means the total sum of k of different latent context features, D means the distortion. The BCE loss is employed to classify whether generated voxels are occupied or not. 
